Improved Online Learning Algorithms for CTR Prediction in Ad Auctions

In this work, we investigate the online learning problem of revenue maximization in ad auctions, where the seller needs to learn the click-through rates (CTRs) of each ad candidate and charge the price of the winner through a pay-per-click manner. We focus on two models of the advertisers' strategic behaviors. First, we assume that the advertiser is completely myopic; i.e.~in each round, they aim to maximize their utility only for the current round. In this setting, we develop an online mechanism based on upper-confidence bounds that achieves a tight $O(\sqrt{T})$ regret in the worst-case and negative regret when the values are static across all the auctions and there is a gap between the highest expected value (i.e.~value multiplied by their CTR) and second highest expected value ad. Next, we assume that the advertiser is non-myopic and cares about their long term utility. This setting is much more complex since an advertiser is incentivized to influence the mechanism by bidding strategically in earlier rounds. In this setting, we provide an algorithm to achieve negative regret for the static valuation setting (with a positive gap), which is in sharp contrast with the prior work that shows $O(T^{2/3})$ regret when the valuation is generated by adversary.

==> non-myopic.tex <==
\section{Non-Myopic Advertisers}\label{sec:non-myopic}
In this section, we consider the  setting that  advertisers behave strategically and aim to maximize their long-term discounted utility. In this setting, advertisers are incentived to  leverage
their private information and “game the system” by submitting (corrupted) bids in an untruthful
and strategic manner so that they can manipulate their predicted clickthrough rates. For example, advertisers may 

For each advertiser $i$, its $\gamma$-discounted long-term expected utility is defined in the following,
\begin{eqnarray}\label{eq:discounted-lt-util}
\ltu_i = \sum_{t=1}^T \gamma^{t-1}\rho_i (v_{i, t} - p_{i, t}) \cdot \ind{i = I_t}
\end{eqnarray}

When $\gamma = 0$, Eq.~\eqref{eq:discounted-lt-util} degenerates to the myopic setting, discussed in the previous section. On the other hand, $\gamma=1$ represents the setting that the advertiser will not discount the future utility.
For the latter setting, \citet{DK09} show $\Omega(T^{2/3})$ regret when the advertisers' valuation are generated adversarially.


\subsection{Adversarial Valuation for Non-Myopic Advertisers with $\gamma < 1$}

To handle the challenge induced by the strategic behaviours of the advertisers, we propose a \emph{phased} algorithm to dampen the advertisers' incentive to mislead the seller and still achieve no-regret guarantee simultaneously. This \emph{phased} algorithm includes multiple phases, where each phase $\ell$ contains $T_\ell$ round. Let $\Gamma_\ell$ denote the set of the rounds in phase $\ell$. To ensure that the non-myopic bidders will not deviate much from the true value, our algorithm enforces some random exploration steps: we pick one of the $n$ buyers uniformly at random with probability $1/T_\ell$ at each round in phase $\ell$, and charge this advertiser with price $r_t\sim \unif[0, 1]$ if its bid $b_t > r_t$ and the ad is clicked. 

\begin{restatable}{lemma}{boundedmisreports}
\label{lem:bounded_misreports}
For each advertiser $i$, define
\begin{eqnarray}
D_{i, \ell} = \left\{t\in \Gamma_\ell: |v_{i,t} - b_{i, t}| \geq \frac{1}{T_\ell}\right\}
\end{eqnarray}
as the set of all rounds in phase $\ell$ during which advertiser $i$ significantly corrupts its bids. Then we have
\begin{eqnarray*}
\Pr\left(|D_{i, \ell}| > \frac{\log(nT^4_\ell)}{\log(1/\gamma)}\right) \leq \frac{1}{T_\ell}
\end{eqnarray*}
\end{restatable}
